BEHAVIOR-1K: A Human-Centered, Embodied AI Benchmark with 1,000 Everyday Activities and Realistic Simulation

We present BEHAVIOR-1K, a comprehensive simulation benchmark for human-centered robotics. BEHAVIOR-1K includes two components, guided and motivated by the results of an extensive survey on "what do you want robots to do for you?". The first is the definition of 1,000 everyday activities, grounded in 50 scenes (houses, gardens, restaurants, offices, etc.) with more than 9,000 objects annotated with rich physical and semantic properties. The second is OMNIGIBSON, a novel simulation environment that supports these activities via realistic physics simulation and rendering of rigid bodies, deformable bodies, and liquids. Our experiments indicate that the activities in BEHAVIOR-1K are long-horizon and dependent on complex manipulation skills, both of which remain a challenge for even state-of-the-art robot learning solutions. To calibrate the simulation-to-reality gap of BEHAVIOR-1K, we provide an initial study on transferring solutions learned with a mobile manipulator in a simulated apartment to its real-world counterpart. We hope that BEHAVIOR-1K's human-grounded nature, diversity, and realism make it valuable for embodied AI and robot learning research. Project website: https://behavior.stanford.edu.

==> T-3-benchmarks-backup.tex <==
% salmon color: 

\begin{table}[!t]
    \definecolor{myGrayCell}{rgb}{.8,.8,.8}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|c|c|c|cccccccccccccccccc|}
        \rot{} & 
        \rot{} & 
        \rot{\textbf{\benchmark}} & 
        \rot{BEHAVIOR-100} & 
        \rot{AI2THOR Vis. Room Rearr.} & 
        \rot{TDW Transport} & 
        \rot{Rearrangement T5 (Habitat)} &
        \rot{ManipulaTHOR ArmPointNav} & 
        \rot{Interactive Gibson Benchmark} & 
        \rot{VirtualHome} & 
        \rot{ALFRED} & 
        \rot{Rearrangement T2 (OCRTOC)} & 
        \rot{IKEA Furniture Assembly} & 
        \rot{RLBench} & 
        \rot{Metaworld} & 
        \rot{Robosuite} & 
        \rot{SoftGym} & 
        \rot{DeepMind Control Suite} & 
        \rot{OpenAIGym} & 
        \rot{Habitat 1.0/2.0} & 
        \rot{Gibson}
        \\\cline{3-21}
        \multicolumn{2}{c}{} & 
        \multicolumn{9}{|c}{Mobile manipulation} & 
        % \multicolumn{2}{|c}{Other planning} & 
        \multicolumn{8}{|c}{Static manipulation} & 
        \multicolumn{2}{|c|}{Navigation}
        \\\cline{2-21}
        
        \rot{} & 
        \multicolumn{1}{|c|}{\begin{tabular}{@{}c@{}}Activities selected\\from human survey\end{tabular}} &
          \textcolor{indiagreen}\faCheck & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes &
         \textcolor{red}\faTimes &
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes 
        \\       
        
        \hline
        & 
         \begin{tabular}{@{}c@{}} Activities\end{tabular} & 
         \textbf{1000} & 
         100 & 
         1 & 
         1 & 
         1 &
         1 & 
         2 & 
         549 & 
          7 & 
         5 & 
         100 & 
         50 & 
         1 & 
         5 & 
         10 & 
         28 & 
         8 & 
         2 & 
         3
        \\

        & 
        \begin{tabular}{@{}c@{}} Scene types \end{tabular} & 
        \textbf{8} & 
        1 & 
        1 & 
        1 &
        1 &
        1 &
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1 & 
        1
        \\
        & 
         Scenes / rooms &
        \begin{tabular}{@{}c@{}}\textbf{50 / }\\\textbf{306}\end{tabular} & 
        \begin{tabular}{@{}c@{}}15 / \\100\end{tabular} & 
        \begin{tabular}{@{}c@{}}- / \\120\end{tabular} & 
        \begin{tabular}{@{}c@{}}15 / \\\end{tabular} & 
        \begin{tabular}{@{}c@{}}55 static / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}- /\\30\end{tabular} & 
        \begin{tabular}{@{}c@{}} 10 /\\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}7 / \\-\end{tabular} &
        \begin{tabular}{@{}c@{}}- / \\120\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}1 / \\-\end{tabular} & 
        \begin{tabular}{@{}c@{}}Matterport\\+ Gibson\end{tabular} &
         \begin{tabular}{@{}c@{}}572\\static\end{tabular}
        \\

        \multirow{3}*{\rotatebox{90}{Diversity}} & 
        % \begin{tabular}{@{}c@{}}Infinite\\-possible sampling\end{tabular} & 
        \begin{tabular}{@{}c@{}}Infinite scene-\\agnostic instantiation\end{tabular} & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        N/A
        \\ 
         & 
         \begin{tabular}{@{}c@{}} Object categories\end{tabular} & 
         \textbf{1224} & 
         391 & 
         118 & 
         ~50 & 
         YCB & 
         150 & 
         5 & 
         509 & 
         84 & 
         12 & 
         73+ & 
         ~28 & 
         7 & 
         10 & 
         4 & 
         4 & 
         4 & 
         Matterport & 
         N/A
        \\
        & 
        \begin{tabular}{@{}c@{}} Object models\end{tabular} & 
        \textbf{3324} & 
        1217 & 
        118 &
        112 & 
        YCB &
        150 & 
        152 & 
        &
        84 &
        101 + YCB & 
        73+ & 
        28 & 
        80 & 
        10 & 
        4 & 
        4 & 
        4 & 
        N/A & 
        N/A
        \\
        % & 
        %  \begin{tabular}{@{}c@{}}\# Object models\\per cat.\end{tabular} & 
        %  \textbf{1-61} & 
        %  1 & 
        %   & 
        %  3 & 
        %  1 & 
        %  12.83 & 
        %  1 & 
        %  1 & 
        %  & 
        %  1 & 
        %  1 & 
        %  1 & 
        %  1 & 
        %  & 
        %  & 
        %  
        % \\
        &
        \begin{tabular}{@{}c@{}} Objs. per activity\end{tabular} & 
        \textbf{3-47} & 
        3-34 & 
        5 &
        7-9 &
        2-5 &
        2-3 & 
        ~10 & 
        1-24 &
        2 &
        5-10 &
        1-2 &
        1-2 &
        1 &
        1-3 &
        1-3 &
        1-3 &
        1 &
        0-1 &
        N/A
        \\        
        
        & 
        \begin{tabular}{@{}c@{}}Diff. state changes required\\per activity \end{tabular} & 
        \textbf{2-11} & 
        2-8 & 
        4 & 
        4 &
        4 &
        2 &
        1-3 & 
        1-7 & 
        2-3 & 
        1 & 
        1-3 & 
        1-4 & 
        4 & 
        1 & 
        1-3 & 
        1-2 & 
        1-2 & 
        1 & 
        1
        \\\cline{1-2}
  


        & 
        \begin{tabular}{@{}c@{}}Kinematics, dynamics\end{tabular} & 
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{red}\faTimes &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck &
        \textcolor{indiagreen}\faCheck 
        \\ 
        \multirow{5}*{\rotatebox{90}{Realism}} & 
         \begin{tabular}{@{}c@{}}Continuous extended\\states (e.g. temp., wetness)\end{tabular} & 
         \textcolor{indiagreen}\faCheck & 
         \textcolor{indiagreen}\faCheck & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes & 
         \textcolor{red}\faTimes 
        \\ 
        & 
        \begin{tabular}{@{}c@{}} Flexible materials\end{tabular} & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes 
        \\ 
        & 
        \begin{tabular}{@{}c@{}}Deformable bodies\end{tabular} & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes 
        \\ 
        & 
        \begin{tabular}{@{}c@{}}Fluid\end{tabular} & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes 
        \\ 
        & 
        \begin{tabular}{@{}c@{}}Fluid dynamics (steam, fire)\end{tabular} & 
        \textcolor{indiagreen}\faCheck & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes & 
        \textcolor{red}\faTimes 
        \\ 
         &
         \begin{tabular}{@{}c@{}}Realistic action execution\end{tabular} & 
         \textcolor{indiagreen}\faCheck &

         \textcolor{indiagreen}\faCheck &
         \textcolor{red}\faTimes &
         \textcolor{indiagreen}\faCheck &
         \textcolor{red}\faTimes &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{red}\faTimes &
         \textcolor{red}\faTimes &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck &
         \textcolor{indiagreen}\faCheck 
        \\
        % & 
        % \begin{tabular}{@{}c@{}}Realistic\\obs. space\end{tabular} &
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{red}\faTimes &
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{indiagreen}\faCheck & 
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{indiagreen}\faCheck 
        % \\
        % & 
        % \begin{tabular}{@{}c@{}}Scenes reconstructed\\from real homes\end{tabular} & 
        % \textcolor{indiagreen} ? &
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{red}\faTimes &
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{red}\faTimes &
        % \textcolor{indiagreen}\faCheck &
        % \textcolor{indiagreen}\faCheck         
        \cline{1-2}

        \rot{} & 
        \multicolumn{1}{|c|}{\begin{tabular}{@{}c@{}}Benchmark focus: Task-\\Planning and/or Control\end{tabular}} & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} TP & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} TP &         
        \cellcolor[rgb]{1,1,1} TP & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} TP+C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} C & 
        \cellcolor[rgb]{1,1,1} C 

        \\\cline{2-21}
    \end{tabular}
  }
  \caption{\textbf{Comparison of Embodied AI Benchmarks:} 
  \benchmark contains 1,000 diverse activities that are grounded by human needs. It achieves a new level of diversity in terms of number of scenes, objects, and state changes involved. \simulator provides realistic simulation of these 1,000 activities, including some of the most advanced simulation and rendering features such as fluid and deformable bodies. [table extended from~\cite{srivastava2021behavior}]}

  \label{tab:comparingbenchmarks}
\end{table}



==> T-6-bak.tex <==
\afterpage{
\clearpage

\begin{table}[H]
\centering
\caption{(two pages) Statistics and information for each of 50 scenes in B1K: scene type, name, number of objects, unique synsets and rooms, room types, and example activities }
\label{tab:model_scene}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|m{0.8cm}|m{4cm}|m{0.6cm}|m{0.6cm}|m{0.6cm}|m{5cm}|m{5cm}|}
\hline
Scene Type
& Scene Name                            & Obj. Cnt.    & Syn. Cnt.    & Rm. Cnt.   & Room Types                                                                                                                                       & Example Activities                                                                                                                                                                                                                 \\ \hline
\multirow{15}{*}{\rotatebox[origin=c]{90}{\textbf{BEHAVIOR-100 Houses}}}
& Beechwood\_0\_int                     & 136          & 32           & 8          & \texttt{bathroom}, \texttt{corridor}, \texttt{dining\_room}, \texttt{entryway}, \texttt{kitchen}, \texttt{living\_room}, \texttt{private\_office}, \texttt{utility\_room}                                                & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Beechwood\_1\_int                     & 129          & 21           & 9          & \texttt{bathroom}, bedroom, childs\_room, closet, \texttt{corridor}, playroom, television\_room                                                                    & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Benevolence\_0\_int                   & 21           & 10           & 4          & \texttt{bathroom}, \texttt{corridor}, empty\_room, \texttt{entryway}                                                                                                        & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Benevolence\_1\_int                   & 74           & 22           & 5          & \texttt{corridor}, \texttt{dining\_room}, \texttt{kitchen}, \texttt{living\_room}, storage\_room                                                                                     & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Benevolence\_2\_int                   & 63           & 23           & 5          & \texttt{bathroom}, bedroom, \texttt{corridor}                                                                                                                      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Ihlen\_0\_int                         & 68           & 21           & 7          & \texttt{bathroom}, \texttt{corridor}, \texttt{dining\_room}, garage, \texttt{living\_room}, storage\_room                                                                            & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Ihlen\_1\_int                         & 147          & 27           & 9          & \texttt{bathroom}, bedroom, \texttt{corridor}, \texttt{dining\_room}, \texttt{kitchen}, \texttt{living\_room}, staircase                                                                      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Merom\_0\_int                         & 82           & 27           & 6          & \texttt{bathroom}, childs\_room, \texttt{living\_room}, playroom, storage\_room, \texttt{utility\_room}                                                                     & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Merom\_1\_int                         & 123          & 28           & 8          & \texttt{bathroom}, bedroom, childs\_room, \texttt{corridor}, \texttt{dining\_room}, \texttt{kitchen}, \texttt{living\_room}, staircase                                                        & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Pomaria\_0\_int                       & 71           & 22           & 6          & \texttt{bathroom}, bedroom, \texttt{corridor}, \texttt{private\_office}, television\_room                                                                                   & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Pomaria\_1\_int                       & 89           & 24           & 6          & \texttt{bathroom}, \texttt{corridor}, \texttt{kitchen}, \texttt{living\_room}, pantry\_room, \texttt{utility\_room}                                                                           & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Pomaria\_2\_int                       & 42           & 18           & 3          & \texttt{bathroom}, bedroom, \texttt{corridor}                                                                                                                      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Rs\_int                               & 72           & 32           & 5          & \texttt{bathroom}, bedroom, \texttt{entryway}, \texttt{kitchen}, \texttt{living\_room}                                                                                               & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Wainscott\_0\_int                     & 187          & 35           & 9          & \texttt{bathroom}, bedroom, \texttt{dining\_room}, \texttt{kitchen}, \texttt{living\_room}                                                                                           & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Wainscott\_1\_int                     & 150          & 26           & 10         & \texttt{bathroom}, bedroom, \texttt{corridor}, exercise\_room, playroom, \texttt{private\_office}, \texttt{utility\_room}                                                            & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\parbox{4cm}{\textbf{BEHAVIOR-100 Houses w/ New Gardens}}}}
& Beechwood\_0\_garden                  & 335          & 45           & 9          & \texttt{bathroom}, \texttt{corridor}, \texttt{dining\_room}, \texttt{entryway}, garden, \texttt{kitchen}, \texttt{living\_room}, \texttt{private\_office}, \texttt{utility\_room}                                        & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Rs\_garden                            & 185          & 47           & 6          & \texttt{bathroom}, bedroom, \texttt{entryway}, garden, \texttt{kitchen}, \texttt{living\_room}                                                                                       & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Pomaria\_0\_garden                    & 260          & 49           & 7          & \texttt{bathroom}, bedroom, \texttt{corridor}, garden, \texttt{private\_office}, television\_room                                                                           & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Merom\_0\_garden                      & 197          & 51           & 8          & \texttt{bathroom}, childs\_room, garden, \texttt{living\_room}, playroom, sauna, storage\_room, \texttt{utility\_room}                                                      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& Wainscott\_0\_garden                  & 712          & 61           & 10         & \texttt{bathroom}, bedroom, \texttt{dining\_room}, garden, \texttt{kitchen}, \texttt{living\_room}                                                                                   & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{New Houses}}}
& house\_single\_floor                  & 1375         & 137          & 23         & \texttt{bathroom}, bedroom, childs\_room, closet, \texttt{corridor}, \texttt{dining\_room}, empty\_room, \texttt{entryway}, garden, \texttt{kitchen}, \texttt{living\_room}, sauna, \texttt{utility\_room}      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& house\_double\_floor\_lower           & 304          & 79           & 6          & \texttt{bathroom}, \texttt{corridor}, garage, garden, \texttt{kitchen}, \texttt{living\_room}                                                                                        & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& house\_double\_floor\_upper           & 325          & 78           & 5          & \texttt{bathroom}, bedroom, television\_room                                                                                                              & example\_activity, example\_activity, example\_activity      \\ \hline
\end{tabular}
}
\end{table}







\begin{table}[H]
\centering
\caption*{Table~\ref{tab:model_scene}, cont'd.}
\resizebox{\textwidth}{!}{%
\setlength\extrarowheight{4pt}
\begin{tabular}{|m{0.8cm}|m{4cm}|m{0.6cm}|m{0.6cm}|m{0.6cm}|m{5cm}|m{5cm}|}
\hline
Scene Type
& Scene Name                            & Obj. Cnt.    & Syn. Cnt.    & Rm. Cnt.   & Room Types                                                                                                                                       & Example Activities                                                                                                                                                                                                                 \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Grocery Stores}}}
& grocery\_store\_asian                 & 3402         & 79           & 2          & \texttt{bathroom}, grocery\_store                                                                                                                         & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& grocery\_store\_cafe                  & 6994         & 71           & 4          & bar, \texttt{bathroom}, \texttt{dining\_room}, grocery\_store                                                                                                      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& grocery\_store\_convenience           & 1889         & 82           & 2          & \texttt{bathroom}, grocery\_store                                                                                                                         & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& grocery\_store\_half\_stocked         & 3804         & 51           & 2          & \texttt{bathroom}, grocery\_store                                                                                                                         & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{Generic Halls}}}
& hall\_arch\_wood                      & 78           & 11           & 2          & \texttt{bathroom}, empty\_room                                                                                                                            & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& hall\_train\_station                  & 141          & 15           & 2          & \texttt{bathroom}, empty\_room                                                                                                                            & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& hall\_glass\_ceiling                  & 116          & 20           & 2          & \texttt{bathroom}, empty\_room                                                                                                                            & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& hall\_conference\_large               & 3372         & 26           & 2          & \texttt{bathroom}, conference\_hall                                                                                                                       & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{Hotels}}}
& hotel\_suite\_large                   & 218          & 51           & 2          & \texttt{bathroom}, bedroom                                                                                                                                & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& hotel\_suite\_small                   & 48           & 28           & 2          & \texttt{bathroom}, bedroom                                                                                                                                & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& hotel\_gym\_spa                       & 322          & 43           & 9          & \texttt{bathroom}, \texttt{corridor}, gym, hammam, locker\_room, sauna, spa                                                                                        & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Offices}}}
& office\_bike                          & 479          & 49           & 3          & \texttt{bathroom}, break\_room, shared\_office                                                                                                            & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& office\_cubicles\_left                & 787          & 44           & 12         & \texttt{bathroom}, conference\_hall, copy\_room, \texttt{corridor}, lobby, meeting\_room, \texttt{private\_office}, shared\_office                                          & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& office\_cubicles\_right               & 406          & 37           & 11         & \texttt{bathroom}, conference\_hall, copy\_room, \texttt{corridor}, lobby, meeting\_room, \texttt{private\_office}, shared\_office                                          & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& office\_large                         & 1151         & 46           & 24         & \texttt{bathroom}, break\_room, conference\_hall, copy\_room, \texttt{corridor}, lobby, meeting\_room, phone\_room, \texttt{private\_office}, shared\_office                & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& office\_vendor\_machine               & 225          & 45           & 4          & \texttt{bathroom}, break\_room, meeting\_room, shared\_office                                                                                             & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{Restaurants}}}
& restaurant\_asian                     & 1221         & 56           & 3          & \texttt{bathroom}, \texttt{dining\_room}, \texttt{kitchen}                                                                                                                  & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& restaurant\_cafeteria                 & 292          & 45           & 3          & \texttt{bathroom}, \texttt{dining\_room}, \texttt{kitchen}                                                                                                                  & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& restaurant\_diner                     & 174          & 39           & 3          & bar, \texttt{bathroom}, \texttt{dining\_room}                                                                                                                      & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& restaurant\_brunch                    & 1096         & 70           & 4          & bar, \texttt{bathroom}, \texttt{dining\_room}, \texttt{kitchen}                                                                                                             & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& restaurant\_urban                     & 1368         & 90           & 4          & bar, \texttt{bathroom}, \texttt{dining\_room}, \texttt{kitchen}                                                                                                             & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& restaurant\_hotel                     & 1080         & 81           & 4          & \texttt{bathroom}, \texttt{dining\_room}, \texttt{kitchen}, lobby                                                                                                           & example\_activity, example\_activity, example\_activity      \\ \hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{Schools}}}
& school\_gym                           & 853          & 36           & 7          & \texttt{bathroom}, \texttt{corridor}, gym, locker\_room                                                                                                            & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& school\_geography                     & 556          & 42           & 5          & \texttt{bathroom}, classroom, \texttt{corridor}                                                                                                                    & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& school\_biology                       & 717          & 53           & 4          & \texttt{bathroom}, biology\_lab, \texttt{corridor}                                                                                                                 & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& school\_chemistry                     & 890          & 69           & 4          & \texttt{bathroom}, chemistry\_lab, \texttt{corridor}                                                                                                               & example\_activity, example\_activity, example\_activity      \\ \cline{2-7} 
& school\_comp\_lab\_infirmary          & 828          & 61           & 6          & \texttt{bathroom}, computer\_lab, \texttt{corridor}, infirmary                                                                                                     & example\_activity, example\_activity, example\_activity      \\ \hline
\end{tabular}
}
\end{table}

}

==> all_activity_table.tex <==
\begin{longtable}{|p{0.3\textwidth}|p{0.3\textwidth}|p{0.3\textwidth}|}
\hline 1. washing floor & 2. cleaning bathrooms & 3. clean your house after a wild party & 4. cleaning floors \\
\hline 
 5. mopping floors & 6. clean a shower & 7. cleaning toilet & 8. cleaning bathtub \\
\hline 
 9. clean grease & 10. scrubbing bathroom floor & 11. cleaning oven & 12. cleaning stove \\
\hline 
 13. shoveling snow & 14. washing outside windows & 15. clean walls & 16. clean up water damage \\
\hline 
 17. washing dishes & 18. vacuuming floors & 19. picking up trash & 20. clean carpets \\
\hline 
 21. emptying trash cans & 22. cleaning pavement & 23. washing plates & 24. washing outside walls \\
\hline 
 25. cleaning windows & 26. sweeping floors & 27. clean the outside of a house & 28. taking trash outside \\
\hline 
 29. clean a couch & 30. washing pots and pans & 31. remove hard water spots & 32. cleaning barbecue grill \\
\hline 
 33. clean a stainless steel dishwasher & 34. sweeping porch & 35. raking leaves & 36. clean cement \\
\hline 
 37. putting dishes away after cleaning & 38. clean your kitty litter box & 39. washing windows & 40. mopping the kitchen floor \\
\hline 
 41. clean outdoor tiles & 42. remove spots from linen & 43. cleaning microwave oven & 44. clean wood siding \\
\hline 
 45. clean a coffee maker & 46. picking up litter & 47. cleaning up after a meal & 48. clean a drain \\
\hline 
 49. clean a sofa & 50. cleaning vehicles & 51. polish wood floors & 52. clean up after a dinner party \\
\hline 
 53. remove ice from gutters & 54. cleaning carpets & 55. sweeping outside entrance & 56. clean mirrors \\
\hline 
 57. clean a broiler pan & 58. vacuuming vehicles & 59. disposing of lawn clippings & 60. cleaning the pool \\
\hline 
 61. unloading shopping from car & 62. waxing cars or other vehicles & 63. clean a grill pan & 64. mowing the lawn \\
\hline 
 65. cleaning up refrigerator & 66. clean your rusty garden tools & 67. removing ice from walkways & 68. cleaning bedroom \\
\hline 
 69. cleaning debris out of car & 70. sweeping garage & 71. wash towels & 72. washing walls \\
\hline 
 73. washing cars or other vehicles & 74. moving stuff to storage & 75. disposing of trash for adult & 76. assembling furniture \\
\hline 
 77. clearing the table after dinner & 78. clean your laundry room & 79. cleaning up after an event & 80. clean an air filter \\
\hline 
 81. tidying bathroom & 82. cleaning up plates and food & 83. installing carpet & 84. cleaning a car \\
\hline 
 85. cleaning the hot tub & 86. moving boxes to storage & 87. clean up gasoline & 88. clean decking \\
\hline 
 89. clean the exterior of your garage & 90. doing laundry & 91. dusting rugs & 92. clean cups \\
\hline 
 93. clean a mattress & 94. shampooing carpet & 95. clean sheets & 96. cleaning up branches and twigs \\
\hline 
 97. waxing floors & 98. clean kitchen appliances & 99. hoe weeds & 100. storing the groceries \\
\hline 
 101. changing sheets & 102. clean rubber bathmats & 103. clean a chicken coop & 104. scraping snow off vehicle \\
\hline 
 105. cleaning patio furniture & 106. cleaning the yard & 107. folding clean laundry & 108. cleaning driveway \\
\hline 
 109. cleaning kitchen cupboard & 110. folding sheets & 111. clean plastic containers & 112. clean a rug \\
\hline 
 113. clean a vacuum & 114. cleaning cupboards & 115. clean your baseboard radiators & 116. clean stainless steel sinks \\
\hline 
 117. clean a glass windshield & 118. clean household cleaning tools & 119. cleaning garden tools & 120. water your lawn efficiently \\
\hline 
 121. ironing clothes & 122. cleaning fan & 123. chop an onion & 124. clean a toaster oven \\
\hline 
 125. disinfect laundry & 126. cleaning up the kitchen only & 127. chopping wood & 128. painting house exterior \\
\hline 
 129. de-clutter your garage & 130. washing utensils & 131. cleaning garage & 132. laying tile floors \\
\hline 
 133. washing fabrics & 134. washing curtains & 135. folding clothes & 136. unpacking moving van \\
\hline 
 137. clean a kitchen sink & 138. shoveling coal & 139. cleaning freezer & 140. putting away yard equipment \\
\hline 
 141. cleaning pet bed & 142. clean a air conditioner & 143. clean out a guinea pigs hutch & 144. clean up broken glass \\
\hline 
 145. clean a rice cooker & 146. polisha car & 147. clean your cleaning supplies & 148. clean a fish \\
\hline 
 149. bringing laundry & 150. applying pesticides & 151. sweeping patio & 152. cleaning shed \\
\hline 
 153. cleaning closet & 154. cleaning table after clearing & 155. putting away Christmas decorations & 156. cleaning parks \\
\hline 
 157. clean a fence & 158. polishing silver & 159. hanging blinds & 160. doing housework for adult \\
\hline 
 161. cleaning the pond & 162. re-shelving library books & 163. clean couch pillows & 164. putting clean laundry away \\
\hline 
 165. rinsing dishes & 166. sweeping steps & 167. polishing furniture & 168. unloading the car \\
\hline 
 169. putting pesticides on lawn & 170. clean an espresso machine & 171. cleaning around pool in garden & 172. clean the interior of your car \\
\hline 
 173. bringing paper to recycling & 174. clean stucco & 175. spraying for bugs & 176. cleaning lawnmowers \\
\hline 
 177. cleaning tools and equipment & 178. laying wood floors & 179. clean a keyboard & 180. putting laundry in drawer \\
\hline 
 181. treating stains & 182. washing bowls & 183. clean a popcorn machine & 184. clean a dirty tent \\
\hline 
 185. clean a baking stone & 186. organizing boxes in garage & 187. clean up spilled egg & 188. changing dog's water \\
\hline 
 189. cleaning boat & 190. clean reusable shopping bags & 191. clean wood doors & 192. dispose of a pizza box \\
\hline 
 193. drying dishes & 194. clean a faucet & 195. prepare a raised bed garden & 196. loading the dishwasher \\
\hline 
 197. clean brass casings & 198. removing lint from dryer & 199. bringing glass to recycling & 200. making the bed \\
\hline 
 201. clean a patio & 202. laying paving stones & 203. clean the bottom of an iron & 204. putting up wallpaper \\
\hline 
 205. fertilize a lawn & 206. cleaning restaurant table & 207. clean an electric razor & 208. lay sod \\
\hline 
 209. clean a hot water dispenser & 210. clean baking sheets & 211. clean a sauna & 212. clean vinyl shutters \\
\hline 
 213. clean a kitchen table & 214. collecting dishes from restaurant tables & 215. delivering groceries to doorstep & 216. clean flip flops \\
\hline 
 217. taking clothes off of the drying rack & 218. cleaning stuff out of car & 219. installing a fence & 220. store firewood \\
\hline 
 221. wash jeans & 222. clean a light bulb & 223. clean rubber & 224. make coffee \\
\hline 
 225. chopping vegetables & 226. fixing broken table & 227. cleaning camper/RV & 228. organise a linen closet \\
\hline 
 229. wash duvets & 230. stock grocery shelves & 231. clean and disinfect ice trays & 232. clean a hamper \\
\hline 
 233. make cabinet doors & 234. replacing screens & 235. tidying living room & 236. clean a box fan \\
\hline 
 237. clean potatoes & 238. carrying in groceries & 239. cleaning garden path & 240. polish copper \\
\hline 
 241. mulching & 242. hanging up curtains & 243. clean a birdcage & 244. de-ice a car \\
\hline 
 245. polishing shoes & 246. loading shopping into car & 247. clearing table after breakfast & 248. remove scorch marks \\
\hline 
 249. cleaning sneakers & 250. hand washing clothing & 251. clearing table after dinner & 252. washing vegetables \\
\hline 
 253. adding chemicals to lawn & 254. dust houseplants & 255. watering outdoor flowers & 256. turning sprinkler off \\
\hline 
 257. dispose of glass & 258. clean a felt pool table top & 259. putting away toys & 260. painting porch \\
\hline 
 261. spraying fruit trees & 262. putting shopping away & 263. cleaning fishing gear & 264. brushing lint off clothing \\
\hline 
 265. clean a blender & 266. stacking wood & 267. loading the car & 268. sanding wood furniture \\
\hline 
 269. clean a toaster & 270. adding chemicals to pool & 271. remove sod & 272. bringing in wood \\
\hline 
 273. clean a sponge & 274. cleaning shoes & 275. clean a piano & 276. store firewood outdoors \\
\hline 
 277. clean a small pet cage & 278. clean brooms & 279. composting waste & 280. getting package from post office \\
\hline 
 281. picking up toys & 282. fertilizing garden & 283. clean quarters & 284. clean a pickup truck \\
\hline 
 285. picking up baggage & 286. recycling office papers & 287. collecting dishes from around house & 288. clean brass \\
\hline 
 289. disinfect nail clippers & 290. putting away Halloween decorations & 291. clearing table after supper & 292. installing appliances \\
\hline 
 293. sorting bottles, cans, and paper & 294. clean a company office & 295. clean a raincoat & 296. lube a bicycle chain \\
\hline 
 297. dispose of paper & 298. clean place mats & 299. clean leather sandals & 300. unloading shopping items \\
\hline 
 301. putting on license plates & 302. fertilize plants & 303. clean cup holders & 304. wash dog toys \\
\hline 
 305. turning sprinkler on & 306. taking clothes out of the dryer & 307. changing bulbs & 308. tidy your garden \\
\hline 
 309. clean wood pallets & 310. clean your electronics & 311. unpacking car for trip & 312. locking every door \\
\hline 
 313. clearing table after snacks & 314. haul a motorcycle & 315. clean a garden sprayer & 316. clean a whiteboard \\
\hline 
 317. recycling newspapers & 318. fill a punching bag & 319. packing moving van & 320. picking up take-out food \\
\hline 
 321. defrosting freezer & 322. line kitchen shelves & 323. clean black rims & 324. recycling glass bottles \\
\hline 
 325. unloading groceries & 326. putting protective cover on vehicle & 327. putting up shelves & 328. sorting laundry \\
\hline 
 329. clean a backpack & 330. carrying out garden furniture & 331. hanging clothes & 332. cleaning glasses off bar \\
\hline 
 333. clean clear plastic & 334. ironing bedsheets & 335. prepare your garden for winter & 336. chlorinating the pool \\
\hline 
 337. hanging clothes on clothesline & 338. putting clothes into closet & 339. putting up Christmas lights outside & 340. clean soot from glass lanterns \\
\hline 
 341. clean a golf club & 342. watering outdoor plants & 343. putting leftovers away & 344. returning consumer goods \\
\hline 
 345. fixing mailbox & 346. hooking up trailer to car & 347. clean a computer monitor & 348. clean pottery \\
\hline 
 349. putting towels in bathroom & 350. clean a dirty baseball & 351. tidying bedroom & 352. repairs to furniture \\
\hline 
 353. cook chicken and rice & 354. clean shrimp & 355. bag groceries & 356. putting dirty dishes in sink \\
\hline 
 357. clean an electric kettle & 358. clean piano keys & 359. cooking food for adult & 360. clean a pizza stone \\
\hline 
 361. collecting wood & 362. putting up Christmas decorations outside & 363. clean gas logs & 364. clean garden gloves \\
\hline 
 365. clean a flat iron & 366. picking up clothes & 367. clean copper wire & 368. remove a broken light bulb \\
\hline 
 369. unpacking recreational vehicle for trip & 370. throwing out used napkins & 371. making photocopies & 372. stripping furniture \\
\hline 
 373. bringing in mail & 374. wash a motorcycle & 375. planting trees & 376. clean clams \\
\hline 
 377. sorting clothing & 378. carrying water & 379. cleaning high chair & 380. turning out all lights before sleep \\
\hline 
 381. cleaning rainboots & 382. covering boat & 383. spray stucco & 384. make pizza \\
\hline 
 385. clean a LED screen & 386. changing light bulbs & 387. brewing coffee & 388. wash your bike \\
\hline 
 389. make pastry & 390. set up a coffee station in your kitchen & 391. putting away tools & 392. clean a gravestone \\
\hline 
 393. clearing table after coffee & 394. polish pewter & 395. thawing frozen food & 396. make ice \\
\hline 
 397. setting mousetraps & 398. clean vases & 399. clean quartz & 400. dispose of batteries \\
\hline 
 401. collect misplaced items & 402. locking every window & 403. cook pasta & 404. clean vans \\
\hline 
 405. can vegetables & 406. ironing curtains & 407. bringing in kindling & 408. putting away cleaning supplies \\
\hline 
 409. folding piece of cloth & 410. installing smoke detectors & 411. clean a quilt & 412. sorting newspapers for recycling \\
\hline 
 413. picking up prescriptions & 414. taking clothes out of washer & 415. putting clothes in storage & 416. reheat frozen or chilled food \\
\hline 
 417. sorting clothes & 418. fixing broken chair & 419. clean an office chair & 420. wash an infant car seat \\
\hline 
 421. hanging up bedsheets & 422. hang icicle lights & 423. organizing items for yard sale & 424. staining wood furniture \\
\hline 
 425. clean a suitcase & 426. returning videotapes to store & 427. putting up outdoor holiday decorations & 428. clean a beer keg \\
\hline 
 429. setting up bedroom for guest & 430. prepare make ahead breakfast bowls & 431. clean a knife block & 432. decorating outside for holidays \\
\hline 
 433. wash baby bottles & 434. sending packages & 435. clean a saxophone & 436. setting the table \\
\hline 
 437. laying restaurant table for dinner & 438. taking clothes off the line & 439. packing boxes for household move or trip & 440. fold towels \\
\hline 
 441. putting in a hot tub & 442. hanging shades & 443. clean a trumpet & 444. clean green beans \\
\hline 
 445. clean a razor blade & 446. clean a bicycle chain & 447. cleaning cups in living room & 448. clean a knife \\
\hline 
 449. clean silver coins & 450. make edible chocolate chip cookie dough & 451. wash lettuce & 452. make instant coffee \\
\hline 
 453. cook fish & 454. clean leather boots & 455. hanging outdoor lights & 456. clean synthetic hiking gear \\
\hline 
 457. organizing file cabinet & 458. unpacking suitcase & 459. clean a lobster & 460. clean sunglasses \\
\hline 
 461. clean a sauna suit & 462. make toast & 463. clean a flat panel monitor & 464. iron curtains \\
\hline 
 465. packing grocery bags into car & 466. packing books into car & 467. make muffins & 468. make pizza dough \\
\hline 
 469. installing a trailer hitch & 470. clean a sieve & 471. make brownies & 472. cook bacon \\
\hline 
 473. prepare baking pans & 474. putting out clean towels & 475. cleaning computer & 476. organizing office documents \\
\hline 
 477. watering indoor flowers & 478. setting up garden furniture & 479. store batteries & 480. clean a wood pipe \\
\hline 
 481. packing cleaning suppies into car & 482. watering houseplants & 483. set up a buffet & 484. planting plants \\
\hline 
 485. wash a bra & 486. set a dinner table & 487. dispose of fireworks & 488. clean oysters \\
\hline 
 489. putting out dog food & 490. clean a mousepad & 491. installing alarms & 492. cook onions \\
\hline 
 493. clean a teddy bear & 494. clean white wall tires & 495. tidying up wardrobe & 496. gathering nuts \\
\hline 
 497. clean a crab & 498. clearing food from table into fridge & 499. putting away purchased clothes & 500. clean copper mugs \\
\hline 
 501. cleaning kitchen knives & 502. clean tennis balls & 503. make chicken fajitas & 504. make soup \\
\hline 
 505. clean a hat & 506. store winter coats & 507. cleaning skis & 508. clean wine glasses \\
\hline 
 509. hanging pictures & 510. store christmas lights & 511. setting up for an event & 512. clean a bowling ball \\
\hline 
 513. wash a wool coat & 514. wash delicates in the laundry & 515. bringing newspaper in & 516. make dinner rolls \\
\hline 
 517. wash goalkeeper gloves & 518. cleaning out drawers & 519. make a small vegetable garden & 520. cooking breakfast \\
\hline 
 521. emptying ashtray & 522. making coffee & 523. make lemon stain remover & 524. treating clothes \\
\hline 
 525. boxing food after dinner & 526. preserving food & 527. clean a tie & 528. clean dog collars \\
\hline 
 529. cook chicken & 530. packing lunches & 531. remove a wall mirror & 532. filling the bird feeder \\
\hline 
 533. clean an iron & 534. putting in a pool & 535. packing fishing gear into car & 536. store rugs \\
\hline 
 537. clean your pencil case & 538. buy pet food for less & 539. slicing vegetables & 540. clean vintage stereo equipment \\
\hline 
 541. cook noodles & 542. thaw frozen fish & 543. make a blended iced cappuccino & 544. buying postage stamps \\
\hline 
 545. store an uncooked turkey & 546. planting flowers & 547. clean nickel & 548. clean fur \\
\hline 
 549. clean tweed & 550. clean batting gloves & 551. boil water & 552. clean a leather belt \\
\hline 
 553. setup a fish tank & 554. prepare a breakfast bar & 555. polish gold & 556. clean white marble \\
\hline 
 557. can syrup & 558. canning food & 559. make cookies & 560. wash fruit and vegetables \\
\hline 
 561. heating soup & 562. putting food in fridge & 563. clean a purse & 564. make batter \\
\hline 
 565. iron a tie & 566. defrost meat & 567. setup a trampoline & 568. clean dentures \\
\hline 
 569. set up two computer monitors & 570. mailing letters & 571. cooking dinner & 572. cooking lunch \\
\hline 
 573. clean prawns & 574. make cake mix & 575. freeze meat & 576. clean a turkey \\
\hline 
 577. rearrange your room & 578. make pizza sauce & 579. putting away games & 580. make nachos \\
\hline 
 581. make a bake sale stand stall & 582. clean paper lampshades & 583. store coffee beans or ground coffee & 584. make popsicles \\
\hline 
 585. polish cymbals & 586. buy boxes for packing & 587. can beans & 588. clean mushrooms \\
\hline 
 589. collecting aluminum cans & 590. puttiing away bicycles & 591. sorting items for garage sale & 592. treating spot \\
\hline 
 593. sorting potatoes & 594. boxing books up for storage & 595. prepare a hanging basket & 596. clean cork mats \\
\hline 
 597. cook rice & 598. clean a pumpkin & 599. hang a dartboard & 600. clean scallops \\
\hline 
 601. storing food & 602. fill a hot water bottle & 603. clean up your desk & 604. heating food up \\
\hline 
 605. fold a cloth napkin & 606. clean jade & 607. clean marker off a doll & 608. grill vegetables \\
\hline 
 609. make fried rice & 610. make an iced espresso & 611. collecting mail from the letterbox & 612. roast vegetables \\
\hline 
 613. clean a watch & 614. make lemon or lime water & 615. store produce & 616. buying cleaning supplies \\
\hline 
 617. clean boxing gloves & 618. praeparing lunch box & 619. planting vegetables & 620. setup a garden party \\
\hline 
 621. clean gourds & 622. make granola & 623. picking vegetables in garden & 624. cook vegetables \\
\hline 
 625. make strawberries and cream & 626. taking down curtains & 627. putting out cat food & 628. organizing volunteer materials \\
\hline 
 629. picking up books at library & 630. clean suede gloves & 631. cook sweet potatoes & 632. wash a leotard \\
\hline 
 633. wash a baseball cap & 634. clean wooden blocks & 635. putting on tags (car) & 636. make cream from milk \\
\hline 
 637. can fruit & 638. prepare and cook prawns & 639. clean your goal keeper gloves & 640. adding fabric softener \\
\hline 
 641. make a cappuccino & 642. sorting household items & 643. clean strawberries & 644. cook ramen noodles \\
\hline 
 645. prepare a filling breakfast & 646. cool cakes & 647. cleaning mushrooms & 648. clean snow peas \\
\hline 
 649. buy home use medical supplies & 650. taking fish out of freezer & 651. making tea & 652. make blueberry mousse \\
\hline 
 653. getting organized for work & 654. making a meal & 655. cook ground beef & 656. preserving vegetables \\
\hline 
 657. make waffles & 658. putting wood in fireplace & 659. putting tablecloth on table & 660. hang a bike on the wall \\
\hline 
 661. make a sugar and coffee scrub & 662. setting up room for a movie & 663. clean snap peas & 664. make a cheese pastry \\
\hline 
 665. make a mojito & 666. wash a backpack & 667. store baby clothes & 668. clean a longboard \\
\hline 
 669. make fish and chips & 670. serving hors d oeuvres & 671. unpacking hobby equipment & 672. cook asparagus \\
\hline 
 673. clean eggs & 674. cook mussels & 675. buy mulch & 676. make iced chocolate \\
\hline 
 677. putting shoes on rack & 678. clean jewels & 679. make applesauce & 680. setting up room for games \\
\hline 
 681. cold brew coffee & 682. make a strawberry slushie & 683. clean a candle jar & 684. cook corn \\
\hline 
 685. rearranging furniture & 686. make a clothes line & 687. cook a brisket & 688. make stew \\
\hline 
 689. turning off the hot tub & 690. baking cookies for the PTA bake sale & 691. cook oysters & 692. grill burgers \\
\hline 
 693. make bagels & 694. throwing away leftovers & 695. drying table & 696. packing hiking equipment into car \\
\hline 
 697. organizing art supplies & 698. buy dog food & 699. make cake filling & 700. installing a printer \\
\hline 
 701. sorting groceries & 702. clean a trombone & 703. packing sports equipment into car & 704. packing art supplies into car \\
\hline 
 705. packing recreational vehicle for trip & 706. putting up posters & 707. cook green beans & 708. make pasta sauce \\
\hline 
 709. prepare your garden for a cat & 710. adding chemicals to hot tub & 711. cook lamb & 712. packing meal for delivery \\
\hline 
 713. turning on radio & 714. make seafood stew & 715. hanging address numbers & 716. glaze a ham \\
\hline 
 717. buying groceries for a feast & 718. collecting berries & 719. cook potatoes & 720. clean baby toys \\
\hline 
 721. make macaroni and cheese & 722. clean geodes & 723. prepare wine and cheese & 724. make a tropical breakfast \\
\hline 
 725. organizing school stuff & 726. rearranging kitchen furniture & 727. attach a camera to a tripod & 728. setting table for coffee \\
\hline 
 729. toast buns & 730. make meatloaf & 731. make tacos & 732. buy rechargeable batteries \\
\hline 
 733. clean mussels & 734. distributing groceries at food bank & 735. filling salt & 736. make baked pears \\
\hline 
 737. installing a scanner & 738. hanging flags & 739. outfit a basic toolbox & 740. drape window scarves \\
\hline 
 741. rack wine & 742. packing food for work & 743. clean seashells & 744. preparing food or drink for sale \\
\hline 
 745. packing car for trip & 746. sorting volunteer materials & 747. cooking a feast & 748. set up a mouse cage \\
\hline 
 749. clean an eraser & 750. clean skateboard bearings & 751. picking fruit and vegetables & 752. cook eggs \\
\hline 
 753. clean pennies & 754. turn off a normal school calculator & 755. toast sunflower seeds & 756. packing child s bag \\
\hline 
 757. make cream soda & 758. pack a pencil case & 759. make lemonade & 760. buy a air conditioner \\
\hline 
 761. clean a book & 762. make oatmeal & 763. serving food on the table & 764. cook spinach \\
\hline 
 765. putting on registration stickers & 766. warm tortillas & 767. roast meat & 768. store beer \\
\hline 
 769. putting up Christmas decorations inside & 770. make chocolate milk & 771. clean cabbage & 772. cook cabbage \\
\hline 
 773. donating clothing & 774. putting up Christmas lights inside & 775. making a drink & 776. make biscuits \\
\hline 
 777. packing hobby equipment & 778. prepare quinoa & 779. buying everyday consumer goods & 780. clean a softball bat \\
\hline 
 781. make chocolate biscuits & 782. hanging up wind chimes & 783. make pumpkin pie spice & 784. make a red meat sauce \\
\hline 
 785. cook squash & 786. decorating outside for parties & 787. buying office supplies & 788. preparing food for adult \\
\hline 
 789. make a milkshake & 790. clean pine cones & 791. clean a glass pipe & 792. turning on the hot tub \\
\hline 
 793. make the workplace exciting & 794. grease and flour a pan & 795. packing picnic food into car & 796. packing documents into car \\
\hline 
 797. cook turkey drumsticks & 798. store loose leaf tea & 799. store feta cheese & 800. packing car for trip \\
\hline 
 801. fold bandanas & 802. sorting art supplies & 803. sorting books on shelf & 804. prepare sea salt soak \\
\hline 
 805. filling pepper & 806. preserving fruit & 807. buying groceries & 808. serving food at a homeless shelter \\
\hline 
 809. clean deer antlers & 810. clean a baseball glove & 811. bringing water & 812. make a salad \\
\hline 
 813. store baking soda & 814. boil water in the microwave & 815. make rose centerpieces & 816. preparing food for company \\
\hline 
 817. cook sausages & 818. clean a loofah or natural sponge & 819. make a sandwich & 820. clean fishing lures \\
\hline 
 821. putting birdseed in cage & 822. put togethera basic pruning kit & 823. cook hot dogs & 824. cook beef and onions \\
\hline 
 825. store tulip bulbs & 826. installing a modem & 827. make fruit punch & 828. prepare an emergency school kit \\
\hline 
 829. store vodka & 830. fill a bucket in a small sink & 831. buy a belt & 832. setup a bar for a cocktail party \\
\hline 
 833. make party favors from candy & 834. sorting mail & 835. set up a webcam & 836. putting bike in garage \\
\hline 
 837. make chicken curry & 838. ice cookies & 839. pour a glass of wine & 840. hard boil an egg \\
\hline 
 841. setup a baby crib & 842. make onion ring batter & 843. setting up living room for guest & 844. donating toys \\
\hline 
 845. cook kale & 846. buy and clean mussels & 847. freeze fruit & 848. pack your gym bag \\
\hline 
 849. make garlic mushrooms & 850. store brownies & 851. making a snack & 852. preparing existing coffee \\
\hline 
 853. opening windows & 854. freeze vegetables & 855. stock a bar & 856. clean greens \\
\hline 
 857. set up a bird cage & 858. opening doors & 859. setting up silent auction & 860. make a wiener schnitzle \\
\hline 
 861. make hot cocoa & 862. cook broccolini & 863. make a frappe & 864. put together a goodie bag \\
\hline 
 865. buy eggs & 866. prepare and cook swiss chard & 867. filling sugar & 868. prepare a slow dinner party \\
\hline 
 869. cook kielbasa & 870. laying clothes out & 871. make a vinegar cleaning solution & 872. freeze lasagna \\
\hline 
 873. cook eggplant & 874. packing child's supplies into car & 875. make cookie dough & 876. set up a hot dog bar \\
\hline 
 877. make king prawns with garlic & 878. clean invisalign & 879. passing out drinks & 880. installing a fax machine \\
\hline 
 881. store a kayak & 882. packing adult s bags & 883. place houseplants around your home & 884. set up a home office in your garage \\
\hline 
 885. make lemon pepper seasoning & 886. buy school supplies for high school & 887. make mustard herb and spice seasoning & 888. cook tofu \\
\hline 
 889. make white wine sauce & 890. cook a turkey & 891. preserving meat & 892. prepare a boat for fishing \\
\hline 
 893. store daffodil bulbs & 894. buy candle making supplies & 895. buy food for a party & 896. set a fancy table \\
\hline 
 897. pack for the pool & 898. wash grapes & 899. pour beer & 900. clean a camera lens \\
\hline 
 901. make watermelon punch & 902. collecting children's toys & 903. cook a frozen pie & 904. make beef and broccoli \\
\hline 
 905. unpacking child's bag & 906. clean a violin & 907. cook shrimp & 908. make stewed fruit \\
\hline 
 909. make red beans and rice & 910. roast nuts & 911. cook kabobs & 912. clean apples \\
\hline 
 913. assembling gift baskets & 914. fold a plastic bag & 915. make limeade & 916. store nuts \\
\hline 
 917. make citrus punch & 918. sautÃ© vegetables & 919. make lemon pepper wings & 920. organizing skating stuff \\
\hline 
 921. preparing food for a fundraiser & 922. cook red peppers & 923. clean bok choy & 924. spring clean your skateboard \\
\hline 
 925. getting a drink & 926. clean whiskey stones & 927. distributing event T-shirts & 928. putting roast in oven \\
\hline 
 929. unhook a fish & 930. make the ultimate spa basket & 931. polish rocks & 932. store a fur coat \\
\hline 
 933. cook mustard greens & 934. make a steak & 935. buy a keg & 936. can meat \\
\hline 
 937. make a christmas gift box & 938. cook clams & 939. mixing drinks & 940. preparing clothes for the next day \\
\hline 
 941. wrap silverware & 942. pack a beach bag & 943. make dinosaur goody bags & 944. make iced tea \\
\hline 
 945. pouring water in a glass & 946. make jamaican jerk seasoning & 947. put together a scrapping tool kit & 948. clean raw denim \\
\hline 
 949. make chocolate spread & 950. freeze quiche & 951. fry pot stickers & 952. selling products at flea market \\
\hline 
 953. arranging home & 954. clean gold & 955. buying fast food & 956. cook brussels sprouts \\
\hline 
 957. cook zucchini & 958. make green tea latte & 959. cook pork ribs & 960. buy good chocolate \\
\hline 
 961. cook quail & 962. store silver coins & 963. make a candy centerpiece & 964. setting the fire \\
\hline 
 965. packing bags or suitcase & 966. make chicken and waffles & 967. make spa water & 968. fold a tortilla \\
\hline 
 969. putting meal in fridge at work & 970. buy a good avocado & 971. clean conch shells & 972. cook a duck \\
\hline 
 973. make chocolate syrup & 974. set up a preschool classroom & 975. cook carrots & 976. make burrito bowls \\
\hline 
 977. cook peppers & 978. cook ham hocks & 979. cover a flower pot in fabric & 980. serving a meal \\
\hline 
 981. paying for purchases & 982. packing picnic into car & 983. buy alcohol & 984. store a quilt \\
\hline 
 985. putting out condiments & 986. make homemade bird food & 987. make tomato rice & 988. make gift bags for baby showers \\
\hline 
 989. clean dentures with vinegar & 990. fill a canteen & 991. set a table for a tea party & 992. make yams \\
\hline 
 993. baking sugar cookies & 994. make bento & 995. bottling fruit & 996. make a basic brine \\
\hline 
 997. cook peas & 998. make cinnamon sugar & 999. halve an egg & 1000. cook a crab \\
\hline 

\caption{All 1,000 \benchmark activities with rank based on human preference score.}
\label{tab:all_activities}
\end{longtable}


==> all_amt_figure.tex <==

\begin{figure}[t]
\captionsetup[subfloat]{labelformat=empty}
\captionsetup[subfloat]{justification=centering}
\centering

\subfloat[\simulator]{}
\hfill
\subfloat[][AI2-Thor]{}
\hfill
\subfloat[][ThreeDWorld]{}
\hfill
\subfloat[][Habitat 2.0]{}
\hfill
\subfloat[][iGibson 2.0]{}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/1.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/1.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/1.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/1.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/1.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/2.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/2.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/2.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/2.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/2.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/3.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/3.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/3.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/3.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/3.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/4.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/4.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/4.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/4.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/4.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/5.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/5.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/5.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/5.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/5.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/6.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/6.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/6.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/6.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/6.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/7.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/7.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/7.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/7.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/7.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/8.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/8.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/8.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/8.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/8.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/9.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/9.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/9.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/9.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/9.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/10.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/10.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/10.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/10.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/10.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/11.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/11.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/11.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/11.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/11.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/12.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/12.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/12.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/12.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/12.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/13.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/13.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/13.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/13.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/13.jpg}}

\end{figure}
% \vspace{-6pt}

\begin{figure}[t]
\captionsetup[subfloat]{labelformat=empty}
\captionsetup[subfloat]{justification=centering}
\centering
% \ContinuedFloat

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/14.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/14.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/14.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/14.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/14.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/15.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/15.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/15.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/15.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/15.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/16.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/16.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/16.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/16.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/16.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/17.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/17.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/17.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/17.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/17.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/18.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/18.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/18.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/18.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/18.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/19.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/19.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/19.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/19.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/19.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/20.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/20.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/20.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/20.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/20.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/21.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/21.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/21.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/21.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/21.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/22.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/22.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/22.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/22.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/22.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/23.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/23.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/23.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/23.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/23.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/24.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/24.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/24.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/24.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/24.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/25.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/25.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/25.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/25.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/25.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/26.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/26.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/26.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/26.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/26.jpg}}

\end{figure}
% \vspace{-6pt}

\begin{figure}[t]
\captionsetup[subfloat]{labelformat=empty}
\captionsetup[subfloat]{justification=centering}
\centering

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/27.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/27.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/27.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/27.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/27.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/28.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/28.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/28.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/28.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/28.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/29.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/29.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/29.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/29.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/29.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/30.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/30.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/30.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/30.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/30.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/31.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/31.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/31.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/31.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/31.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/32.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/32.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/32.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/32.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/32.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/33.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/33.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/33.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/33.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/33.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/34.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/34.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/34.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/34.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/34.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/35.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/35.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/35.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/35.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/35.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/36.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/36.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/36.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/36.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/36.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/37.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/37.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/37.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/37.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/37.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/38.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/38.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/38.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/38.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/38.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/39.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/39.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/39.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/39.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/39.jpg}}

\end{figure}
% \vspace{-6pt}

\begin{figure}[t]
\captionsetup[subfloat]{labelformat=empty}
\captionsetup[subfloat]{justification=centering}
\centering

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/40.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/40.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/40.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/40.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/40.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/41.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/41.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/41.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/41.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/41.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/42.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/42.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/42.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/42.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/42.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/43.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/43.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/43.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/43.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/43.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/44.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/44.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/44.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/44.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/44.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/45.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/45.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/45.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/45.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/45.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/46.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/46.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/46.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/46.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/46.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/47.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/47.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/47.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/47.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/47.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/48.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/48.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/48.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/48.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/48.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/49.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/49.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/49.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/49.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/49.jpg}}

\vspace{-6pt}

\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/og/50.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ai2/50.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/tdw/50.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/habitat/50.jpg}}
\hfill
\subfloat[][]{\includegraphics[width=.199\textwidth]{figures/omnigibson/amt_study/ig2/50.jpg}}



\vspace{15pt}
\caption{\textbf{Comparative Evaluation of Visual Realism:} We evaluate \simulator's visual realism against other simulation environments by running a survey with 50 human participants. We ask them to rank the realism of sampled images from each environment with a score of 5 (most realistic) to 1 (least realistic). We report the mean and standard deviation and show a sampled image from the study. We observe that the participants consider \simulator to be significantly more visually realistic than all other environments. See Appendix \ref{amt_study_appx} for more info.}
\label{fig:sim_render}
\end{figure}
